Robust Beamforming for RIS-aided Communications: Gradient-based Manifold Meta Learning

Reconfigurable intelligent surface (RIS) has become a promising technology to realize the programmable wireless environment via steering the incident signal in fully customizable ways. However, a major challenge in RIS-aided communication systems is the simultaneous design of the precoding matrix at the base station (BS) and the phase shifting matrix of the RIS elements. This is mainly attributed to the highly non-convex optimization space of variables at both the BS and the RIS, and the diversity of communication environments. Generally, traditional optimization methods for this problem suffer from the high complexity, while existing deep learning based methods are lack of robustness in various scenarios. To address these issues, we introduce a gradient-based manifold meta learning method (GMML), which works without pre-training and has strong robustness for RIS-aided communications. Specifically, the proposed method fuses meta learning and manifold learning to improve the overall spectral efficiency, and reduce the overhead of the high-dimensional signal process. Unlike traditional deep learning based methods which directly take channel state information as input, GMML feeds the gradients of the precoding matrix and phase shifting matrix into neural networks. Coherently, we design a differential regulator to constrain the phase shifting matrix of the RIS. Numerical results show that the proposed GMML can improve the spectral efficiency by up to 7.31\%, and speed up the convergence by 23 times faster compared to traditional approaches. Moreover, they also demonstrate remarkable robustness and adaptability in dynamic settings.

==> baseline.tex <==
\section{Alternating Optimization Method}\label{sec:baseline}
Alternating optimization (AO) algorithms typically use the non-convex block coordinate descent (BCD) method. This approach involves breaking down optimization variables into multiple blocks, updating each block according to specific rules while keeping the remaining blocks fixed at their most recently updated values. For RIS-assisted communications, the optimization problem is divided into two sub-problems. The first focuses on the conventional beamforming design problem at the BS, while the second addresses the phase optimization problem at the RIS.

\subsection{Algorithm Description}
When $\mathbf{\Theta}$ is temporarily held fixed , the problem reduces to the SE maximization problem for the conventional MU-MISO system, which has been thoroughly investigated. One of the best-known solutions is WMMSE, which provides closed-form expression and can deliver high performance. If the cascaded channel of user $k$ is expressed as $\mathbf{h}_{c,k}=\mathbf{h}^H_k \mathbf{\Theta G} \in \mathbb{C}^{1 \times M}$, the iterative updating rule can be expressed in the following manner

\begin{subequations}
\begin{align}
u_k &= \left(\sum_{i=1}^{K} |\mathbf{h}^H_{c,k}\mathbf{w}_i|^2 + \sigma^2 \right)^{-1}\mathbf{h}^H_{c,k}\mathbf{w}_k,  \\
\Omega_k &= \left(1 - u_k^* \mathbf{h}^H_{c,k}\mathbf{w}_k  \right)^{-1}, \\
\mathbf{w}_k &= \omega_k u_k \Omega_k\left(\lambda\mathbf{I}_M + \sum_{i=1}^{K}\omega_i|u_i|^2\Omega_i\mathbf{h}_{c,i}\mathbf{h}_{c,i}^H\right)^{-1}\mathbf{h}_{c,i},
\end{align}
\end{subequations}
in which $\lambda$ serves as the dual parameter for the power constraint, and typically the bisection method is utilized to determine the optimal parameter.
\par
When keeping $\mathbf{W}$ temporarily fixed, the focus can be shifted to the phase optimization problem. The Riemannian conjugate gradient (RCG) algorithm is a suitable solution for this problem due to the constraint forming a complex circle manifold. We can define the effective channel and RIS phase as
\begin{equation}
    \mathbf{a}_{i,k} = \mathrm{diag} (\mathbf{h}_{k}^H)\mathbf{G}\mathbf{w}_i,
\end{equation}
\begin{equation}
    \mathbf{\theta}= [e^{j\theta_1}, e^{j\theta_2}, \cdots, e^{j\theta_N}]^H,
\end{equation}
and the phase optimization problem can be represented as 

\begin{equation}
\begin{split}
& R(\mathbf{\Theta}) =\mathop{\max}_{\theta} \sum_{k=1}^{K}\omega_k \log (1 + \frac{|\mathbf{\theta}^H\mathbf{a}_{k,k}|^2}{\sum_{i \neq k}|\mathbf{\theta}^H\mathbf{a}_{i,k}|^2+\sigma^2}), \\
& \mathrm{s.t.} \quad |\mathbf{\theta}_n|=1, \forall n=1,\dots,N.
\end{split}
\end{equation}
To perform RCG algorithm, we must first compute the Riemannian gradient, which is the orthogonal projection of the Euclidean gradient $\nabla R$ on the complex circle
\begin{equation}
    \mathrm{grad} R = \nabla R - \mathrm{Re}\{\nabla R \circ \mathbf{\theta}^*\}\circ \mathbf{\theta},
\end{equation}
where the Euclidean gradient is
\begin{equation}
   \nabla R = \sum_{k=1}^K2\omega_k\mathbf{S}_k,
\end{equation}
and $\mathbf{S}_k$ can be expressed as
\begin{equation}
   \mathbf{S}_k = \frac{\sum_i\mathbf{a}_{i,k}\mathbf{a}_{i,k}^H\mathbf{\theta}}{\sum_i|\mathbf{\theta}^H\mathbf{a}_{i,k}|^2 + \sigma^2} - \frac{\sum_{i \neq k}\mathbf{a}_{i,k}\mathbf{a}_{i,k}^H\mathbf{\theta}}{\sum_{i \neq k}|\mathbf{\theta}^H\mathbf{a}_{i,k}|^2 + \sigma^2}.
\end{equation}
Then the search direction can be found by the tangent vector conjugate to $\nabla R$
\begin{equation}
    \mathbf{d} = -\nabla R + \eta_1 T(\overline{\mathbf{d}}).
\end{equation}
$\eta_1$ is the conjugate gradient update parameter, and $\overline{\mathbf{d}}$ is the previous search direction.
After acquiring the tangent vector, we need to project it to the complex circle manifold as
\begin{equation}
    \mathbf{\theta}_{n + 1} = \frac{(\mathbf{\theta}+ \eta_2\mathbf{d})_n}{|(\mathbf{\theta}+ \eta_2 \mathbf{d})_n|},
\end{equation}
where $\eta_2$ denotes the Armijo step size.


\subsection{Discussion}
The aforementioned straightforward BCD algorithm is combined with the WMMSE algorithm and the RCG algorithm, which function iteratively and independently in solving the NP-hard problem. The WMMSE algorithm is known to have a complexity $\mathcal{O}(L_1 K M^3)$, where $L_1$ represents the total number of WMMSE convergence iterations. While the RCG algorithm has a complexity $\mathcal{O}(L_2 K^2 N^2)$, where $L_2$ represents the total number of RCG convergence iterations. Thus the total complexity is $\mathcal{O}(L_3(L_1 K M^3 + L_2 K^2 N^2))$, where $L_3$ denotes the total number of outer loops. This complexity is noticeably high, as it is cubic in the number of antennas and quadratic in both the number of RIS components and users, leading to significant overhead.



